Constrained Serial Dictatorships can be Fair

When allocating indivisible items to agents, it is known that the only strategyproof mechanisms that satisfy a set of rather mild conditions are constrained serial dictatorships: given a fixed order over agents, at each step the designated agent chooses a given number of items (depending on her position in the sequence). Agents who come earlier in the sequence have a larger choice of items; however, this advantage can be compensated by a higher number of items received by those who come later. How to balance priority in the sequence and number of items received is a nontrivial question. We use a previous model, parameterized by a mapping from ranks to scores, a social welfare functional, and a distribution over preference profiles. For several meaningful choices of parameters, we show that the optimal sequence can be computed exactly in polynomial time or approximated using sampling. Our results hold for several probabilistic models on preference profiles, with an emphasis on the Plackett-Luce model. We conclude with experimental results showing how the optimal sequence is impacted by various parameters.

==> macros.tex <==
\NewEnviron{cproblem}[1]{%
\begin{center}\fbox{\parbox{3in}{%
    {\centering\scshape #1\par}%
    \parskip=1ex
    %\everypar{\hangindent=1em}%
    \BODY
}}\end{center}}

\NewEnviron{cproblemArxiv}[1]{%
\begin{center}\fbox{\parbox{6in}{%
    {\centering\scshape #1\par}%
    \parskip=1ex
    %\everypar{\hangindent=1em}%
    \BODY
}}\end{center}}

\newcommand{\AgentSet}{\mathcal{A}}
\newcommand{\ItemSet}{\mathcal{I}}
\newcommand{\PickingSequence}{\pi}
\newcommand{\AllocationFunction}[2]{\phi_{#1}^{#2}}
\newcommand{\ProbModel}{\Psi}
\newcommand{\Rank}{\mathtt{rk}}
\newcommand{\FI}{\mathtt{FI}}
\newcommand{\FC}{\mathtt{FC}}
\newcommand{\FIC}[1]{\FI\text{-}\FC_{#1}}
\newcommand{\MM}[1]{\mathtt{M}_{#1}}
\newtheorem{observation}{Observation}
\newtheorem{observationApp}{Observation$^*$}
\newtheorem{condition}{Condition}
\newtheorem{lemma}{Lemma}
\newtheorem{lemmaApp}{Lemma$^*$}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{propositionApp}{Proposition$^*$}
\usepackage{amsfonts}

\newcommand{\HG}[1]{{\color{red}[HG : #1]}}
\newcommand{\sylvain}[1]{{\color{cyan}[Sylvain: #1]}} 
\newcommand{\jerome}[1]{{\color{purple}[Jerome : #1]}} 
\newcommand{\fjerome}[1]{\endnote{\color{purple}[Jerome : #1]}}
\newcommand{\fsylvain}[1]{\endnote{\color{cyan}[Sylvain]}}
\newcommand{\fMG}[1]{\endnote{\color{blue}[Guillaume]}}
\newcommand{\fHG}[1]{\endnote{\color{red}[HG : #1]}}
\newcommand{\MG}[1]{{\color{blue}[Guillaume: #1]}} 

==> packages.tex <==
\usepackage{environ}
\usepackage{endnotes}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}
\usepackage{thmtools} 
\usepackage{thm-restate}
\usepackage[lite]{mtpro2}

==> plots.tex <==
%\subsection{Number of objects picked per agents}
%Borda

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda and egalitarian social welfare}
    title={egalitarian},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_Borda_egalitarian.txt};
}
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and utilitarian social welfare }
    title={utilitarian},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_Borda_utilitarian.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={nash},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_Borda_nash.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda and egalitarian social welfare}
    title={egalitarian,Lexi},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_Lexicographic_egalitarian.txt};
}
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and utilitarian social welfare }
    title={utilitarian,Lexi},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_Lexicographic_utilitarian.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={nash,Lexi},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_Lexicographic_nash.txt};
}
\end{axis}

\end{tikzpicture}



\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda and egalitarian social welfare}
    title={egalitarian,QI : eps = 5e-2},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_QI5e-2_egalitarian.txt};
}
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and utilitarian social welfare }
    title={utilitarian,QI : eps = 5e-2},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_QI5e-2_utilitarian.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={nash,QI : eps = 5e-2},
    xlabel={Number of objects available},
    ylabel={Number of objetcs picked}
]
\foreach \n in{0,...,14}{
    \addplot table[x=m, y=Nb\n] {./Data/15_200_QI5e-2_nash.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={utilitarian Borda},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Borda_utilitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={egalitarian Borda},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Borda_egalitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={nash Borda},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Borda_nashnb_obj.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={utilitarian harmonique},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Harmonique_utilitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={egalitarian harmonique},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Harmonique_egalitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={nash Harmonique},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Harmonique_nashnb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={utilitarian Anti-harmonique},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Anti_Harmonique_utilitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={egalitarian Anti-harmonique},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Anti_Harmonique_egalitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    %title={Number of objects picked by agents for 15 agents sharing 15 to 200 objects, with Borda vector and Nash social welfare },
    title={nash Anti-harmonique},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/15_200_Anti_Harmonique_nashnb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    title={utilitarian Borda2},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_utilitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    title={egalitarian Borda2},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_egalitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    title={nash Borda2},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_nashnb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\newpage

\begin{tikzpicture}
\begin{axis}[
    title={utilitarian borda2},
    xlabel={Agent},
    ylabel={Utility}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_utilitarian_uti.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    title={egalitarian Borda2},
    xlabel={Agent},
    ylabel={Utility}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_egalitarian_uti.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    title={nash Borda2},
    xlabel={Agent},
    ylabel={Utility}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_nash_uti.txt};
}
\end{axis}

\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    title={utilitarian Borda},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda_utilitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}



\begin{tikzpicture}
\begin{axis}[
    title={egalitarian Borda},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda_egalitariannb_obj.txt};
}
\end{axis}

\end{tikzpicture}




\begin{tikzpicture}
\begin{axis}[
    title={nash Borda},
    xlabel={Agent},
    ylabel={Number of object picked}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda_nashnb_obj.txt};
}
\end{axis}

\end{tikzpicture}

\newpage

\begin{tikzpicture}
\begin{axis}[
    title={utilitarian Borda},
    xlabel={Agent},
    ylabel={Utility}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda_utilitarian_uti.txt};
}
\end{axis}

\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    title={egalitarian Borda},
    xlabel={Agent},
    ylabel={Utility}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_egalitarian_uti.txt};
}
\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    title={nash Borda},
    xlabel={Agent},
    ylabel={Utility}
]
\foreach \n in{1,...,10}{
    \addplot table[x index=0, y index=\n] {./Data/5_300_Borda2_nash_uti.txt};
}
\end{axis}

\end{tikzpicture}


\newpage


